It's not a Non-Issue: Negation as a Source of Error in Machine Translation

As machine translation (MT) systems progress at a rapid pace, questions of their adequacy linger. In this study we focus on negation, a universal, core property of human language that significantly affects the semantics of an utterance. We investigate whether translating negation is an issue for modern MT systems using 17 translation directions as test bed. Through thorough analysis, we find that indeed the presence of negation can significantly impact downstream quality, in some cases resulting in quality reductions of more than 60%. We also provide a linguistically motivated analysis that directly explains the majority of our findings. We release our annotations and code to replicate our analysis here: https://github.com/mosharafhossain/negation-mt.

==> tables/da_bleu_meteor.tex <==
\begin{tabular}{r@{ $\rightarrow$ }l rr rr rr}
\toprule

\multicolumn{2}{c}{} & \multicolumn{2}{c}{Z vs. BLEU} & \multicolumn{2}{c}{Z vs. chrF++} & \multicolumn{2}{c}{Z vs. METEOR} \\
  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
\multicolumn{2}{c}{} & w/ neg. & w/o neg. & w/ neg. & w/o neg. & w/ neg. & w/o neg. \\

\midrule

ru & en & 0.420 & 0.714 & 0.508 & 0.736 & 0.464 & 0.604 \\ \hline
de & en & 0.483 & 0.633 & 0.517 & 0.600 & 0.517 & 0.567 \\ \hline
fi & en & 0.788 & 0.818 & 0.848 & 0.909 & 0.879 & 0.758 \\ \hline
lt & en & 0.709 & 0.796 & 0.673 & 0.796 & 0.709 & 0.796 \\ \hline
gu & en & 0.564 & 0.745 & 0.782 & 0.964 & 0.527 & 0.891 \\ \hline
kk & en & 0.855 & 0.818 & 0.673 & 0.855 & 0.745 & 0.782 \\ \hline

\end{tabular}

\iffalse
\begin{tabular}{|l||c|c||c|c||c|c|}
\hline
                           & \multicolumn{2}{c||}{Z-score vs. BLEU} & \multicolumn{2}{c||}{Z-score vs. chrF++} &
                             \multicolumn{2}{c|}{Z-score vs. METEOR} \\ \cline{2-7}
                           & w/ neg. & w/o neg. &
                             w/ neg. & w/o neg. & 
                             w/ neg. & w/o neg. \\ \hline
ru $\rightarrow$ en      & 0.420* & 0.714* & 0.508* & 0.736* & 0.464* & 0.604* \\ \hline
de $\rightarrow$ en      & 0.483* & 0.633* & 0.517* & 0.600* & 0.517* & 0.567* \\ \hline
fi $\rightarrow$ en      & 0.788 & 0.818 & 0.848 & 0.909 & 0.879 & 0.758 \\ \hline
lt $\rightarrow$ en      & 0.709* & 0.796* & 0.673* & 0.796* & 0.709* & 0.796* \\ \hline
gu $\rightarrow$ en      & 0.564 & 0.745 & 0.782 & 0.964 & 0.527 & 0.891 \\ \hline
kk $\rightarrow$ en      & 0.855* & 0.818* & 0.673* & 0.855* & 0.745* & 0.782* \\ \hline

\end{tabular}
\fi


==> tex/background.tex <==
\section{Related Work}\label{sec:background}

\an{I don't like related work sections, and I prefer to include the necessary references throughout the text. That said, if you'd like to have one, I won't object :) How about a negation 101 section? -- For a standard related work section, though, I'd put this section before the conclusion, to not tire the reader and break the flow of the paper.}

\ap{yep, fine with me. I like the idea of Negation 101!}

==> tex/questions.tex <==
\begin{enumerate}

\item Compare human scores of the best system for each language direction:
(a) all sentences (absolute)
and
(b) sentences with negation (absolute and relative wrt (a))
    and sentences without negation (absolute and relative wrt (a)).
We expect sentences with negation to have lower scores for many language pairs (Table \ref{t:best_all}).

\paragraph{Comparing z-scores with and without negation}


\item Compare rankings of all systems for all language directions (Kendall's Tau) using
all sentences and sentences with negation.
We expect the rankings to change (Table \ref{t:ranking_all}).

\item Illustrate actual rank differences.
  For each language direction: ranking evaluating with all sentences, ranking evaluating with sentences with negation, and ranking evaluating with sentences without negation. Include in the paper one or two directions with the highest lowest Kendall's Tau, the rest in supplementary materials (Table \ref{t:ranking_one_pair}).
  
\item (not sure) Compare the rankings (Kendall's Tau)
using human scores, BLEU and METEOR when calculated with
all sentences, sentences with negation and sentences without negation.
Are BLEU and METEOR equally good with sentences with negation and without negation? (Table \ref{t:da_bleu_meteor})

\item Correlation between absolute scores
(a) with sentences without negation (or all sentences?)
and
(b) with sentence with negation.
Do systems translate sentences with negation bad regardless of overall scoring? (Figure \ref{f:all_diff}

\item Correlation between
(a) similarity score between language pairs
and
(b) drop in scores (all sentences vs. sentences with negation) (Figure \ref{f:similarity_diff}).

\item Divergence distributions per language (similar to previous analysis by AA). Align the negation cues, and figure out how far the differences between reference and system translations are (close: it is just the cue; far away: wider implications, will need to investigate). Before or after the cue?

\item Qualitative analysis.
  \begin{enumerate}
  \item Why are negations easier and harder to translate in some languages? (theoretical point of view?)
  \item For selected language pairs (X-en), look at the reference and system translations with negation. What is the problem? Meaning is lost? Opposite? Syntax / grammar?
  \item (maybe) For selected language pairs, look at the tokens aligned to the English negation cue. Are there interesting patterns related to the language and its properties wrt negation? Are there interesting patterns related to the type of negation cue on the English side?
  \end{enumerate}

\end{enumerate}
